A Framework for Integrating Gesture Generation Models into Interactive Conversational Agents

Embodied conversational agents (ECAs) benefit from non-verbal behavior for natural and efficient interaction with users. Gesticulation - hand and arm movements accompanying speech - is an essential part of non-verbal behavior. Gesture generation models have been developed for several decades: starting with rule-based and ending with mainly data-driven methods. To date, recent end-to-end gesture generation methods have not been evaluated in a real-time interaction with users. We present a proof-of-concept framework, which is intended to facilitate evaluation of modern gesture generation models in interaction. We demonstrate an extensible open-source framework that contains three components: 1) a 3D interactive agent; 2) a chatbot backend; 3) a gesticulating system. Each component can be replaced, making the proposed framework applicable for investigating the effect of different gesturing models in real-time interactions with different communication modalities, chatbot backends, or different agent appearances. The code and video are available at the project page https://nagyrajmund.github.io/project/gesturebot.

==> sections/2related_work.tex <==
\section{Related work}
\subsection{Gesticulating conversational agents}

%While traditional , 
The nonverbal behavior of currently existing embodied conversational agents often includes gesticulation \cite{lhommet2015cerebella, matsuyama2016socially, rodriguez2016singing, Le2012CoSpeechNao}, typically specified in the Behavior Markup Language (BML) \cite{kopp2006towards} format. One example is Cerebella \cite{lhommet2015cerebella}, an interactive virtual agent where head movements, eye gaze and gesture animations are generated from speech. SARA (Socially-Aware Robot Assistant) from Matsuyama et al. \cite{matsuyama2016socially} is a personal assistant that analyses the user's speech along with their head and face movement in order to build and maintain dyadic rapport. %It uses a nonverbal behavior generator called BEAT \cite{cassell2004beat}, which outputs the gestures in BML as well.
Recently, Rodriges et al.~\cite{rodriguez2016singing} have developed an interactive system enabling NAO robots to gesticulate while talking.

While these agents are capable of producing high quality gestures, they utilize rule-based methods and hence they cannot fully capture the richness of human gesticulation. %\textbf{\textcolor{magenta}{Can we state this as a fact? Does it need evidence? (How) should we rephrase it? - Rajmund}}

\subsection{Gesture generation}
Gesture generation for embodied agents has been an active research field for several decades \cite{levine2010gesture, chiu2015predicting, sadoughi2019speech, kucherenko2019analyzing, yoon2019robots, alexanderson2020style}. Due to space constraints, we limit ourselves to the data-driven methods and review only a subset of them. Levine et al. \cite{levine2010gesture} proposed a system which could produce convincing gestures selected from a gesture library in real-time from audio prosody features. Later Chiu et al.~\cite{chiu2015predicting} proposed a model to generate gesture class given speech audio, text and part-of-speech. Sadoughi et al.~\cite{sadoughi2019speech} proposed a model to generate gesture categories from speech conditioned on a discourse function. Most of these methods \cite{levine2010gesture, chiu2015predicting, sadoughi2019speech} could produce only a discrete set of gestures. Only since recently it is possible to generate continuous arbitrary gestures in a data-driven way from speech audio \cite{alexanderson2020style, kucherenko2019analyzing}, text \cite{yoon2019robots} and the combination of the two~\cite{kucherenko2020gesticulator}.

To the best of our knowledge, this paper is the first to integrate one of the latest end-to-end gesture generation methods into a conversational agent. 

%That is what we have done in this paper.

% A BIT TOO POMPOUS. We aim to bring the two communities together and let ECA researcher have an easy access to the latest gesture generation models.
